Suppression of charged particle production at large transverse momentum in central Pb-Pb collisions at $\sqrt{s_{\rm NN}} = 2.76$ TeV

Inclusive transverse momentum spectra of primary charged particles in Pb-Pb collisions at $\sqrt{s_{_{\rm NN}}}$ = 2.76 TeV have been measured by the ALICE Collaboration at the LHC. The data are presented for central and peripheral collisions, corresponding to 0-5% and 70-80% of the hadronic Pb-Pb cross section. The measured charged particle spectra in $|\eta|<0.8$ and $0.3 < p_T < 20$ GeV/$c$ are compared to the expectation in pp collisions at the same $\sqrt{s_{\rm NN}}$, scaled by the number of underlying nucleon-nucleon collisions. The comparison is expressed in terms of the nuclear modification factor $R_{\rm AA}$. The result indicates only weak medium effects ($R_{\rm AA} \approx $ 0.7) in peripheral collisions. In central collisions, $R_{\rm AA}$ reaches a minimum of about 0.14 at $p_{\rm T}=6$-7GeV/$c$ and increases significantly at larger $p_{\rm T}$. The measured suppression of high-$p_{\rm T}$ particles is stronger than that observed at lower collision energies, indicating that a very dense medium is formed in central Pb-Pb collisions at the LHC.

==> authors-Elsarticle.tex <==
% Author list created by c:\users\kuijer\documents\visual studio 2010\projects\aliautorlist\aliautorlist\alixmldocument.cpp(Nov 21 2010)
% XML file: file:///C:/Documents and Settings/kuijer/Documents/Visual Studio 2010/Projects/AliAutorList/AliAutorList/authors-2010-11-27.xml
% XML created on: 2010-11-27T11:00:17
% merged with: 
%           file:///C:/Documents and Settings/kuijer/Documents/Visual Studio 2010/Projects/AliAutorList/AliAutorList/authors-exceptions-until2011.xml
%
\author[a1]{K.~Aamodt}
\author[a2]{A.~Abrahantes~Quintana}
\author[a3]{D.~Adamov\'{a}}
\author[a4]{A.M.~Adare}
\author[a5]{M.M.~Aggarwal}
\author[a6]{G.~Aglieri~Rinella}
\author[a7]{A.G.~Agocs}
\author[a8]{S.~Aguilar~Salazar}
\author[a9]{Z.~Ahammed}
\author[a10]{N.~Ahmad}
\author[a10]{A.~Ahmad~Masoodi}
\author[a11]{S.U.~Ahn\fnref{f1}}
\author[a12]{A.~Akindinov}
\author[a13]{D.~Aleksandrov}
\author[a14]{B.~Alessandro}
\author[a8]{R.~Alfaro~Molina}
\author[a15]{A.~Alici\fnref{f2}}
\author[a16]{A.~Alkin}
\author[a8]{E.~Almar\'az~Avi\~na}
\author[a17]{T.~Alt}
\author[a18]{V.~Altini}
\author[a19]{S.~Altinpinar}
\author[a20]{I.~Altsybeev}
\author[a21]{C.~Andrei}
\author[a19]{A.~Andronic}
\author[a22]{V.~Anguelov\fnref{f3, 4}}
\author[a23]{C.~Anson}
\author[a24]{T.~Anti\v{c}i\'{c}}
\author[a25]{F.~Antinori}
\author[a26]{P.~Antonioli}
\author[a27]{L.~Aphecetche}
\author[a28]{H.~Appelsh\"{a}user}
\author[a29]{N.~Arbor}
\author[a15]{S.~Arcelli}
\author[a28]{A.~Arend}
\author[a30]{N.~Armesto}
\author[a14]{R.~Arnaldi}
\author[a4]{T.~Aronsson}
\author[a19]{I.C.~Arsene}
\author[a20]{A.~Asryan}
\author[a6]{A.~Augustinus}
\author[a19]{R.~Averbeck}
\author[a31]{T.C.~Awes}
\author[a32]{J.~\"{A}yst\"{o}}
\author[a10]{M.D.~Azmi}
\author[a17]{M.~Bach}
\author[a33]{A.~Badal\`{a}}
\author[a11]{Y.W.~Baek\fnref{f1}}
\author[a14]{S.~Bagnasco}
\author[a28]{R.~Bailhache}
\author[a34]{R.~Bala\fnref{f5}}
\author[a35]{R.~Baldini~Ferroli}
\author[a36]{A.~Baldisseri}
\author[a37]{A.~Baldit}
\author[a38]{J.~B\'{a}n}
\author[a39]{R.~Barbera}
\author[a18]{F.~Barile}
\author[a7]{G.G.~Barnaf\"{o}ldi}
\author[a40]{L.S.~Barnby}
\author[a37]{V.~Barret}
\author[a41]{J.~Bartke}
\author[a15]{M.~Basile}
\author[a37]{N.~Bastid}
\author[a42]{B.~Bathen}
\author[a27]{G.~Batigne}
\author[a43]{B.~Batyunya}
\author[a28]{C.~Baumann}
\author[a44]{I.G.~Bearden}
\author[a28]{H.~Beck}
\author[a45]{I.~Belikov}
\author[a15]{F.~Bellini}
\author[a46]{R.~Bellwied\fnref{f6}}
\author[a8]{\mbox{E.~Belmont-Moreno}}
\author[a34]{S.~Beole}
\author[a21]{I.~Berceanu}
\author[a21]{A.~Bercuci}
\author[a19]{E.~Berdermann}
\author[a47]{Y.~Berdnikov}
\author[a6]{L.~Betev}
\author[a48]{A.~Bhasin}
\author[a5]{A.K.~Bhati}
\author[a34]{L.~Bianchi}
\author[a49]{N.~Bianchi}
\author[a25]{C.~Bianchin}
\author[a50]{J.~Biel\v{c}\'{\i}k}
\author[a3]{J.~Biel\v{c}\'{\i}kov\'{a}}
\author[a51]{A.~Bilandzic}
\author[a34]{E.~Biolcati}
\author[a37]{A.~Blanc}
\author[a52]{F.~Blanco}
\author[a53]{F.~Blanco}
\author[a13]{D.~Blau}
\author[a28]{C.~Blume}
\author[a6]{M.~Boccioli}
\author[a23]{N.~Bock}
\author[a54]{A.~Bogdanov}
\author[a44]{H.~B{\o}ggild}
\author[a55]{M.~Bogolyubsky}
\author[a7]{L.~Boldizs\'{a}r}
\author[a56]{M.~Bombara}
\author[a25]{C.~Bombonati}
\author[a28]{J.~Book}
\author[a36]{H.~Borel}
\author[a25]{C.~Bortolin\fnref{f7}}
\author[a57]{S.~Bose}
\author[a34]{F.~Boss\'u}
\author[a51]{M.~Botje}
\author[a22]{S.~B\"{o}ttger}
\author[a58]{B.~Boyer}
\author[a19]{\mbox{P.~Braun-Munzinger}}
\author[a59]{L.~Bravina}
\author[a60]{M.~Bregant\fnref{f8}}
\author[a22]{T.~Breitner}
\author[a61]{M.~Broz}
\author[a6]{R.~Brun}
\author[a4]{E.~Bruna}
\author[a18]{G.E.~Bruno}
\author[a62]{D.~Budnikov}
\author[a28]{H.~Buesching}
\author[a63]{O.~Busch}
\author[a64]{Z.~Buthelezi}
\author[a25]{D.~Caffarri}
\author[a65]{X.~Cai}
\author[a4]{H.~Caines}
\author[a66]{E.~Calvo~Villar}
\author[a60]{P.~Camerini}
\author[a6]{V.~Canoa~Roman\fnref{f9, 10}}
\author[a26]{G.~Cara~Romeo}
\author[a6]{F.~Carena}
\author[a6]{W.~Carena}
\author[a6]{F.~Carminati}
\author[a49]{A.~Casanova~D\'{\i}az}
\author[a6]{M.~Caselle}
\author[a36]{J.~Castillo~Castellanos}
\author[a21]{V.~Catanescu}
\author[a6]{C.~Cavicchioli}
\author[a14]{P.~Cerello}
\author[a32]{B.~Chang}
\author[a6]{S.~Chapeland}
\author[a36]{J.L.~Charvet}
\author[a57]{S.~Chattopadhyay}
\author[a9]{S.~Chattopadhyay}
\author[a67]{M.~Cherney}
\author[a68]{C.~Cheshkov}
\author[a68]{B.~Cheynis}
\author[a14]{E.~Chiavassa}
\author[a6]{V.~Chibante~Barroso}
\author[a69]{D.D.~Chinellato}
\author[a6]{P.~Chochula}
\author[a70]{M.~Chojnacki}
\author[a70]{P.~Christakoglou}
\author[a44]{C.H.~Christensen}
\author[a71]{P.~Christiansen}
\author[a72]{T.~Chujo}
\author[a73]{C.~Cicalo}
\author[a15]{L.~Cifarelli}
\author[a26]{F.~Cindolo}
\author[a64]{J.~Cleymans}
\author[a35]{F.~Coccetti}
\author[a45]{J.-P.~Coffin}
\author[a14]{S.~Coli}
\author[a49]{G.~Conesa~Balbastre\fnref{f11}}
\author[a27]{Z.~Conesa~del~Valle\fnref{f12}}
\author[a63]{P.~Constantin}
\author[a60]{G.~Contin}
\author[a74]{J.G.~Contreras}
\author[a46]{T.M.~Cormier}
\author[a34]{Y.~Corrales~Morales}
\author[a75]{I.~Cort\'{e}s~Maldonado}
\author[a76]{P.~Cortese}
\author[a69]{M.R.~Cosentino}
\author[a6]{F.~Costa}
\author[a52]{M.E.~Cotallo}
\author[a74]{E.~Crescio}
\author[a37]{P.~Crochet}
\author[a77]{E.~Cuautle}
\author[a49]{L.~Cunqueiro}
\author[a18]{G.~D~Erasmo}
\author[a78]{A.~Dainese\fnref{f13}}
\author[a44]{H.H.~Dalsgaard}
\author[a79]{A.~Danu}
\author[a57]{D.~Das}
\author[a57]{I.~Das}
\author[a80]{A.~Dash}
\author[a14]{S.~Dash}
\author[a9]{S.~De}
\author[a49]{A.~De~Azevedo~Moregula}
\author[a81]{G.O.V.~de~Barros}
\author[a82]{A.~De~Caro}
\author[a83]{G.~de~Cataldo}
\author[a17]{J.~de~Cuveland}
\author[a84]{A.~De~Falco}
\author[a82]{D.~De~Gruttola}
\author[a14]{N.~De~Marco}
\author[a82]{S.~De~Pasquale}
\author[a14]{R.~De~Remigis}
\author[a70]{R.~de~Rooij}
\author[a27]{H.~Delagrange}
\author[a66]{Y.~Delgado~Mercado}
\author[a76]{G.~Dellacasa\fnref{f14}}
\author[a85]{A.~Deloff}
\author[a62]{V.~Demanov}
\author[a7]{E.~D\'{e}nes}
\author[a81]{A.~Deppman}
\author[a18]{D.~Di~Bari}
\author[a18]{C.~Di~Giglio}
\author[a86]{S.~Di~Liberto}
\author[a6]{A.~Di~Mauro}
\author[a49]{P.~Di~Nezza}
\author[a42]{T.~Dietel}
\author[a6]{R.~Divi\`{a}}
\author[a1]{{\O}.~Djuvsland}
\author[a46]{A.~Dobrin\fnref{f15}}
\author[a85]{T.~Dobrowolski}
\author[a77]{I.~Dom\'{\i}nguez}
\author[a19]{B.~D\"{o}nigus}
\author[a59]{O.~Dordic}
\author[a27]{O.~Driga}
\author[a9]{A.K.~Dubey}
\author[a6]{J.~Dubuisson}
\author[a68]{L.~Ducroux}
\author[a37]{P.~Dupieux}
\author[a57]{A.K.~Dutta~Majumdar}
\author[a9]{M.R.~Dutta~Majumdar}
\author[a83]{D.~Elia}
\author[a42]{D.~Emschermann}
\author[a22]{H.~Engel}
\author[a87]{H.A.~Erdal}
\author[a58]{B.~Espagnon}
\author[a27]{M.~Estienne}
\author[a72]{S.~Esumi}
\author[a40]{D.~Evans}
\author[a6]{S.~Evrard}
\author[a59]{G.~Eyyubova}
\author[a6]{C.W.~Fabjan\fnref{f16}}
\author[a88]{D.~Fabris}
\author[a29]{J.~Faivre}
\author[a15]{D.~Falchieri}
\author[a49]{A.~Fantoni}
\author[a19]{M.~Fasel}
\author[a64]{R.~Fearick}
\author[a43]{A.~Fedunov}
\author[a1]{D.~Fehlker}
\author[a61]{V.~Fekete}
\author[a79]{D.~Felea}
\author[a20]{G.~Feofilov}
\author[a75]{A.~Fern\'{a}ndez~T\'{e}llez}
\author[a34]{A.~Ferretti}
\author[a76]{R.~Ferretti\fnref{f17}}
\author[a81]{M.A.S.~Figueredo}
\author[a62]{S.~Filchagin}
\author[a83]{R.~Fini}
\author[a89]{D.~Finogeev}
\author[a18]{F.M.~Fionda}
\author[a18]{E.M.~Fiore}
\author[a6]{M.~Floris}
\author[a64]{S.~Foertsch}
\author[a19]{P.~Foka}
\author[a13]{S.~Fokin}
\author[a90]{E.~Fragiacomo}
\author[a91]{M.~Fragkiadakis}
\author[a19]{U.~Frankenfeld}
\author[a6]{U.~Fuchs}
\author[a6]{F.~Furano}
\author[a29]{C.~Furget}
\author[a82]{M.~Fusco~Girard}
\author[a44]{J.J.~Gaardh{\o}je}
\author[a29]{S.~Gadrat}
\author[a34]{M.~Gagliardi}
\author[a66]{A.~Gago}
\author[a34]{M.~Gallio}
\author[a91]{P.~Ganoti\fnref{f18}}
\author[a19]{C.~Garabatos}
\author[a76]{R.~Gemme}
\author[a17]{J.~Gerhard}
\author[a27]{M.~Germain}
\author[a36]{C.~Geuna}
\author[a6]{A.~Gheata}
\author[a6]{M.~Gheata}
\author[a18]{B.~Ghidini}
\author[a9]{P.~Ghosh}
\author[a92]{M.R.~Girard}
\author[a14]{G.~Giraudo}
\author[a34]{P.~Giubellino\fnref{f19}}
\author[a41]{\mbox{E.~Gladysz-Dziadus}}
\author[a63]{P.~Gl\"{a}ssel}
\author[a93]{R.~Gomez}
\author[a8]{\mbox{L.H.~Gonz\'{a}lez-Trueba}}
\author[a52]{\mbox{P.~Gonz\'{a}lez-Zamora}}
\author[a75]{H.~Gonz\'{a}lez~Santos}
\author[a17]{S.~Gorbunov}
\author[a94]{S.~Gotovac}
\author[a8]{V.~Grabski}
\author[a63]{R.~Grajcarek}
\author[a70]{A.~Grelli}
\author[a6]{A.~Grigoras}
\author[a6]{C.~Grigoras}
\author[a54]{V.~Grigoriev}
\author[a95]{A.~Grigoryan}
\author[a43]{S.~Grigoryan}
\author[a16]{B.~Grinyov}
\author[a90]{N.~Grion}
\author[a71]{P.~Gros}
\author[a6]{\mbox{J.F.~Grosse-Oetringhaus}}
\author[a68]{J.-Y.~Grossiord}
\author[a88]{R.~Grosso}
\author[a89]{F.~Guber}
\author[a29]{R.~Guernane}
\author[a66]{C.~Guerra~Gutierrez}
\author[a15]{B.~Guerzoni}
\author[a44]{K.~Gulbrandsen}
\author[a96]{T.~Gunji}
\author[a48]{A.~Gupta}
\author[a48]{R.~Gupta}
\author[a19]{H.~Gutbrod}
\author[a1]{{\O}.~Haaland}
\author[a58]{C.~Hadjidakis}
\author[a79]{M.~Haiduc}
\author[a96]{H.~Hamagaki}
\author[a7]{G.~Hamar}
\author[a4]{J.W.~Harris}
\author[a28]{M.~Hartig}
\author[a49]{D.~Hasch}
\author[a79]{D.~Hasegan}
\author[a26]{D.~Hatzifotiadou}
\author[a95]{A.~Hayrapetyan\fnref{f17}}
\author[a42]{M.~Heide}
\author[a4]{M.~Heinz}
\author[a87]{H.~Helstrup}
\author[a21]{A.~Herghelegiu}
\author[a19]{C.~Hern\'{a}ndez}
\author[a74]{G.~Herrera~Corral}
\author[a63]{N.~Herrmann}
\author[a87]{K.F.~Hetland}
\author[a4]{B.~Hicks}
\author[a4]{P.T.~Hille}
\author[a45]{B.~Hippolyte}
\author[a72]{T.~Horaguchi}
\author[a96]{Y.~Hori}
\author[a6]{P.~Hristov}
\author[a58]{I.~H\v{r}ivn\'{a}\v{c}ov\'{a}}
\author[a1]{M.~Huang}
\author[a19]{S.~Huber}
\author[a23]{T.J.~Humanic}
\author[a97]{D.S.~Hwang}
\author[a27]{R.~Ichou}
\author[a62]{R.~Ilkaev}
\author[a85]{I.~Ilkiv}
\author[a72]{M.~Inaba}
\author[a84]{E.~Incani}
\author[a34]{G.M.~Innocenti}
\author[a6]{P.G.~Innocenti}
\author[a13]{M.~Ippolitov}
\author[a10]{M.~Irfan}
\author[a19]{C.~Ivan}
\author[a20]{A.~Ivanov}
\author[a19]{M.~Ivanov}
\author[a47]{V.~Ivanov}
\author[a6]{A.~Jacho{\l}kowski}
\author[a98]{P.M.~Jacobs}
\author[a43]{L.~Jancurov\'{a}}
\author[a45]{S.~Jangal}
\author[a61]{R.~Janik}
\author[a53]{S.P.~Jayarathna\fnref{f20}}
\author[a99]{S.~Jena}
\author[a6]{L.~Jirden}
\author[a40]{G.T.~Jones}
\author[a40]{P.G.~Jones}
\author[a40]{P.~Jovanovi\'{c}}
\author[a11]{H.~Jung}
\author[a11]{W.~Jung}
\author[a40]{A.~Jusko}
\author[a17]{S.~Kalcher}
\author[a38]{P.~Kali\v{n}\'{a}k}
\author[a42]{M.~Kalisky}
\author[a32]{T.~Kalliokoski}
\author[a100]{A.~Kalweit}
\author[a70]{R.~Kamermans\fnref{f14}}
\author[a1]{K.~Kanaki}
\author[a11]{E.~Kang}
\author[a101]{J.H.~Kang}
\author[a54]{V.~Kaplin}
\author[a89]{O.~Karavichev}
\author[a89]{T.~Karavicheva}
\author[a89]{E.~Karpechev}
\author[a13]{A.~Kazantsev}
\author[a22]{U.~Kebschull}
\author[a102]{R.~Keidel}
\author[a10]{M.M.~Khan}
\author[a47]{A.~Khanzadeev}
\author[a55]{Y.~Kharlov}
\author[a87]{B.~Kileng}
\author[a32]{D.J.~Kim}
\author[a11]{D.S.~Kim}
\author[a11]{D.W.~Kim}
\author[a11]{H.N.~Kim}
\author[a97]{J.H.~Kim}
\author[a11]{J.S.~Kim}
\author[a11]{M.~Kim}
\author[a101]{M.~Kim}
\author[a97]{S.~Kim}
\author[a11]{S.H.~Kim}
\author[a6]{S.~Kirsch\fnref{f21}}
\author[a22]{I.~Kisel\fnref{f4}}
\author[a12]{S.~Kiselev}
\author[a6]{A.~Kisiel}
\author[a103]{J.L.~Klay}
\author[a63]{J.~Klein}
\author[a42]{C.~Klein-B\"{o}sing}
\author[a28]{M.~Kliemant}
\author[a1]{A.~Klovning}
\author[a6]{A.~Kluge}
\author[a19]{M.L.~Knichel}
\author[a63]{K.~Koch}
\author[a19]{M.K.~K\"{o}hler}
\author[a59]{R.~Kolevatov}
\author[a20]{A.~Kolojvari}
\author[a20]{V.~Kondratiev}
\author[a54]{N.~Kondratyeva}
\author[a89]{A.~Konevskih}
\author[a41]{E.~Korna\'{s}}
\author[a46]{C.~Kottachchi~Kankanamge~Don}
\author[a40]{R.~Kour}
\author[a41]{M.~Kowalski}
\author[a29]{S.~Kox}
\author[a13]{K.~Kozlov}
\author[a32]{J.~Kral}
\author[a38]{I.~Kr\'{a}lik}
\author[a28]{F.~Kramer}
\author[a100]{I.~Kraus\fnref{f22}}
\author[a63]{T.~Krawutschke\fnref{f23}}
\author[a17]{M.~Kretz}
\author[a40]{M.~Krivda\fnref{f24}}
\author[a63]{D.~Krumbhorn}
\author[a50]{M.~Krus}
\author[a47]{E.~Kryshen}
\author[a51]{M.~Krzewicki}
\author[a13]{Y.~Kucheriaev}
\author[a45]{C.~Kuhn}
\author[a51]{P.G.~Kuijer}
\author[a85]{P.~Kurashvili}
\author[a89]{A.~Kurepin}
\author[a89]{A.B.~Kurepin}
\author[a62]{A.~Kuryakin}
\author[a3]{S.~Kushpil}
\author[a3]{V.~Kushpil}
\author[a63]{M.J.~Kweon}
\author[a101]{Y.~Kwon}
\author[a39]{P.~La~Rocca}
\author[a52]{P.~Ladr\'{o}n~de~Guevara\fnref{f25}}
\author[a58]{V.~Lafage}
\author[a22]{C.~Lara}
\author[a1]{D.T.~Larsen}
\author[a40]{C.~Lazzeroni}
\author[a58]{Y.~Le~Bornec}
\author[a60]{R.~Lea}
\author[a11]{K.S.~Lee}
\author[a11]{S.C.~Lee}
\author[a27]{F.~Lef\`{e}vre}
\author[a28]{J.~Lehnert}
\author[a6]{L.~Leistam}
\author[a27]{M.~Lenhardt}
\author[a83]{V.~Lenti}
\author[a93]{I.~Le\'{o}n~Monz\'{o}n}
\author[a28]{H.~Le\'{o}n~Vargas}
\author[a7]{P.~L\'{e}vai}
\author[a104]{X.~Li}
\author[a40]{R.~Lietava}
\author[a59]{S.~Lindal}
\author[a22]{V.~Lindenstruth\fnref{f4}}
\author[a6]{C.~Lippmann\fnref{f22}}
\author[a23]{M.A.~Lisa}
\author[a1]{L.~Liu}
\author[a46]{V.R.~Loggins}
\author[a54]{V.~Loginov}
\author[a6]{S.~Lohn}
\author[a63]{D.~Lohner}
\author[a37]{X.~Lopez}
\author[a58]{M.~L\'{o}pez~Noriega}
\author[a2]{E.~L\'{o}pez~Torres}
\author[a59]{G.~L{\o}vh{\o}iden}
\author[a63]{X.-G.~Lu}
\author[a28]{P.~Luettig}
\author[a25]{M.~Lunardon}
\author[a34]{G.~Luparello}
\author[a27]{L.~Luquin}
\author[a6]{C.~Luzzi}
\author[a65]{K.~Ma}
\author[a4]{R.~Ma}
\author[a53]{D.M.~Madagodahettige-Don}
\author[a89]{A.~Maevskaya}
\author[a6]{M.~Mager}
\author[a80]{D.P.~Mahapatra}
\author[a45]{A.~Maire}
\author[a47]{M.~Malaev}
\author[a77]{I.~Maldonado~Cervantes}
\author[a12]{D.~Mal'Kevich}
\author[a19]{P.~Malzacher}
\author[a62]{A.~Mamonov}
\author[a37]{L.~Manceau}
\author[a48]{L.~Mangotra}
\author[a13]{V.~Manko}
\author[a37]{F.~Manso}
\author[a83]{V.~Manzari}
\author[a65]{Y.~Mao\fnref{f26}}
\author[a105]{J.~Mare\v{s}}
\author[a60]{G.V.~Margagliotti}
\author[a26]{A.~Margotti}
\author[a19]{A.~Mar\'{\i}n}
\author[a106]{I.~Martashvili}
\author[a6]{P.~Martinengo}
\author[a75]{M.I.~Mart\'{\i}nez}
\author[a8]{A.~Mart\'{\i}nez~Davalos}
\author[a27]{G.~Mart\'{\i}nez~Garc\'{\i}a}
\author[a16]{Y.~Martynov}
\author[a27]{A.~Mas}
\author[a19]{S.~Masciocchi}
\author[a34]{M.~Masera}
\author[a73]{A.~Masoni}
\author[a68]{L.~Massacrier}
\author[a83]{M.~Mastromarco}
\author[a6]{A.~Mastroserio}
\author[a40]{Z.L.~Matthews}
\author[a41]{A.~Matyja\fnref{f8}}
\author[a77]{D.~Mayani}
\author[a14]{G.~Mazza}
\author[a86]{M.A.~Mazzoni}
\author[a107]{F.~Meddi}
\author[a8]{\mbox{A.~Menchaca-Rocha}}
\author[a6]{P.~Mendez~Lorenzo}
\author[a63]{J.~Mercado~P\'erez}
\author[a14]{P.~Mereu}
\author[a72]{Y.~Miake}
\author[a108]{J.~Midori}
\author[a34]{L.~Milano}
\author[a59]{J.~Milosevic\fnref{f27}}
\author[a70]{A.~Mischke}
\author[a19]{D.~Mi\'{s}kowiec\fnref{f19}}
\author[a79]{C.~Mitu}
\author[a46]{J.~Mlynarz}
\author[a9]{B.~Mohanty}
\author[a6]{L.~Molnar}
\author[a74]{L.~Monta\~{n}o~Zetina}
\author[a14]{M.~Monteno}
\author[a52]{E.~Montes}
\author[a25]{M.~Morando}
\author[a81]{D.A.~Moreira~De~Godoy}
\author[a25]{S.~Moretto}
\author[a6]{A.~Morsch}
\author[a49]{V.~Muccifora}
\author[a94]{E.~Mudnic}
\author[a6]{H.~M\"{u}ller}
\author[a9]{S.~Muhuri}
\author[a81]{M.G.~Munhoz}
\author[a75]{J.~Munoz}
\author[a6]{L.~Musa}
\author[a14]{A.~Musso}
\author[a99]{B.K.~Nandi}
\author[a26]{R.~Nania}
\author[a83]{E.~Nappi}
\author[a106]{C.~Nattrass}
\author[a18]{F.~Navach}
\author[a40]{S.~Navin}
\author[a9]{T.K.~Nayak}
\author[a62]{S.~Nazarenko}
\author[a62]{G.~Nazarov}
\author[a12]{A.~Nedosekin}
\author[a68]{F.~Nendaz}
\author[a109]{J.~Newby}
\author[a18]{M.~Nicassio}
\author[a44]{B.S.~Nielsen}
\author[a13]{S.~Nikolaev}
\author[a24]{V.~Nikolic}
\author[a13]{S.~Nikulin}
\author[a47]{V.~Nikulin}
\author[a67]{B.S.~Nilsen}
\author[a59]{M.S.~Nilsson}
\author[a26]{F.~Noferini}
\author[a70]{G.~Nooren}
\author[a32]{N.~Novitzky}
\author[a13]{A.~Nyanin}
\author[a99]{A.~Nyatha}
\author[a44]{C.~Nygaard}
\author[a1]{J.~Nystrand}
\author[a108]{H.~Obayashi}
\author[a20]{A.~Ochirov}
\author[a100]{H.~Oeschler}
\author[a11]{S.K.~Oh}
\author[a92]{J.~Oleniacz}
\author[a14]{C.~Oppedisano}
\author[a77]{A.~Ortiz~Velasquez}
\author[a34]{G.~Ortona}
\author[a71]{A.~Oskarsson}
\author[a92]{P.~Ostrowski}
\author[a71]{I.~Otterlund}
\author[a19]{J.~Otwinowski}
\author[a1]{G.~{\O}vrebekk}
\author[a63]{K.~Oyama}
\author[a96]{K.~Ozawa}
\author[a63]{Y.~Pachmayer}
\author[a50]{M.~Pachr}
\author[a34]{F.~Padilla}
\author[a82]{P.~Pagano}
\author[a77]{G.~Pai\'{c}}
\author[a17]{F.~Painke}
\author[a30]{C.~Pajares}
\author[a36]{S.~Pal}
\author[a9]{S.K.~Pal}
\author[a40]{A.~Palaha}
\author[a33]{A.~Palmeri}
\author[a33]{G.S.~Pappalardo}
\author[a19]{W.J.~Park}
\author[a83]{V.~Paticchio}
\author[a46]{A.~Pavlinov}
\author[a92]{T.~Pawlak}
\author[a70]{T.~Peitzmann}
\author[a13]{D.~Peresunko}
\author[a51]{C.E.~P\'erez~Lara}
\author[a6]{D.~Perini}
\author[a18]{D.~Perrino}
\author[a92]{W.~Peryt}
\author[a26]{A.~Pesci}
\author[a6]{V.~Peskov}
\author[a110]{Y.~Pestov}
\author[a6]{A.J.~Peters}
\author[a50]{V.~Petr\'{a}\v{c}ek}
\author[a21]{M.~Petris}
\author[a40]{P.~Petrov}
\author[a21]{M.~Petrovici}
\author[a39]{C.~Petta}
\author[a90]{S.~Piano}
\author[a14]{A.~Piccotti}
\author[a61]{M.~Pikna}
\author[a27]{P.~Pillot}
\author[a6]{O.~Pinazza}
\author[a53]{L.~Pinsky}
\author[a28]{N.~Pitz}
\author[a6]{F.~Piuz}
\author[a46]{D.B.~Piyarathna\fnref{f28}}
\author[a40]{R.~Platt}
\author[a98]{M.~P\l{}osko\'{n}}
\author[a92]{J.~Pluta}
\author[a43]{T.~Pocheptsov\fnref{f29}}
\author[a7]{S.~Pochybova}
\author[a93]{P.L.M.~Podesta-Lerma}
\author[a34]{M.G.~Poghosyan}
\author[a105]{K.~Pol\'{a}k}
\author[a55]{B.~Polichtchouk}
\author[a21]{A.~Pop}
\author[a50]{V.~Posp\'{\i}\v{s}il}
\author[a48]{B.~Potukuchi}
\author[a46]{S.K.~Prasad\fnref{f30}}
\author[a35]{R.~Preghenella}
\author[a14]{F.~Prino}
\author[a46]{C.A.~Pruneau}
\author[a89]{I.~Pshenichnov}
\author[a84]{G.~Puddu}
\author[a39]{A.~Pulvirenti}
\author[a62]{V.~Punin}
\author[a56]{M.~Puti\v{s}}
\author[a4]{J.~Putschke}
\author[a6]{E.~Quercigh}
\author[a59]{H.~Qvigstad}
\author[a90]{A.~Rachevski}
\author[a6]{A.~Rademakers}
\author[a6]{O.~Rademakers}
\author[a63]{S.~Radomski}
\author[a32]{T.S.~R\"{a}ih\"{a}}
\author[a32]{J.~Rak}
\author[a36]{A.~Rakotozafindrabe}
\author[a76]{L.~Ramello}
\author[a74]{A.~Ram\'{\i}rez~Reyes}
\author[a42]{M.~Rammler}
\author[a111]{R.~Raniwala}
\author[a111]{S.~Raniwala}
\author[a32]{S.S.~R\"{a}s\"{a}nen}
\author[a106]{K.F.~Read}
\author[a29]{J.S.~Real}
\author[a85]{K.~Redlich}
\author[a28]{R.~Renfordt}
\author[a49]{A.R.~Reolon}
\author[a89]{A.~Reshetin}
\author[a17]{F.~Rettig}
\author[a6]{J.-P.~Revol}
\author[a63]{K.~Reygers}
\author[a100]{H.~Ricaud}
\author[a14]{L.~Riccati}
\author[a78]{R.A.~Ricci}
\author[a1]{M.~Richter\fnref{f31}}
\author[a6]{P.~Riedler}
\author[a6]{W.~Riegler}
\author[a39]{F.~Riggi}
\author[a14]{A.~Rivetti}
\author[a75]{M.~Rodr\'{i}guez~Cahuantzi}
\author[a17]{D.~Rohr}
\author[a1]{D.~R\"ohrich}
\author[a19]{R.~Romita}
\author[a49]{F.~Ronchetti}
\author[a6]{P.~Rosinsk\'{y}}
\author[a37]{P.~Rosnet}
\author[a6]{S.~Rossegger}
\author[a25]{A.~Rossi}
\author[a91]{F.~Roukoutakis}
\author[a58]{S.~Rousseau}
\author[a27]{C.~Roy\fnref{f12}}
\author[a57]{P.~Roy}
\author[a52]{A.J.~Rubio~Montero}
\author[a60]{R.~Rui}
\author[a6]{I.~Rusanov}
\author[a13]{E.~Ryabinkin}
\author[a41]{A.~Rybicki}
\author[a55]{S.~Sadovsky}
\author[a6]{K.~\v{S}afa\v{r}\'{\i}k}
\author[a25]{R.~Sahoo}
\author[a80]{P.K.~Sahu}
\author[a6]{P.~Saiz}
\author[a98]{S.~Sakai}
\author[a72]{D.~Sakata}
\author[a30]{C.A.~Salgado}
\author[a9]{T.~Samanta}
\author[a48]{S.~Sambyal}
\author[a47]{V.~Samsonov}
\author[a38]{L.~\v{S}\'{a}ndor}
\author[a8]{A.~Sandoval}
\author[a72]{M.~Sano}
\author[a96]{S.~Sano}
\author[a42]{R.~Santo}
\author[a83]{R.~Santoro}
\author[a32]{J.~Sarkamo}
\author[a37]{P.~Saturnini}
\author[a26]{E.~Scapparone}
\author[a25]{F.~Scarlassara}
\author[a112]{R.P.~Scharenberg}
\author[a21]{C.~Schiaua}
\author[a63]{R.~Schicker}
\author[a19]{C.~Schmidt}
\author[a19]{H.R.~Schmidt}
\author[a6]{S.~Schreiner}
\author[a28]{S.~Schuchmann}
\author[a6]{J.~Schukraft}
\author[a27]{Y.~Schutz\fnref{f17}}
\author[a19]{K.~Schwarz}
\author[a63]{K.~Schweda}
\author[a15]{G.~Scioli}
\author[a14]{E.~Scomparin}
\author[a40]{P.A.~Scott}
\author[a106]{R.~Scott}
\author[a25]{G.~Segato}
\author[a76]{S.~Senyukov}
\author[a11]{J.~Seo}
\author[a84]{S.~Serci}
\author[a52]{E.~Serradilla}
\author[a79]{A.~Sevcenco}
\author[a43]{G.~Shabratova}
\author[a6]{R.~Shahoyan}
\author[a5]{N.~Sharma}
\author[a48]{S.~Sharma}
\author[a108]{K.~Shigaki}
\author[a72]{M.~Shimomura}
\author[a2]{K.~Shtejer}
\author[a13]{Y.~Sibiriak}
\author[a34]{M.~Siciliano}
\author[a6]{E.~Sicking}
\author[a85]{T.~Siemiarczuk}
\author[a15]{A.~Silenzi}
\author[a31]{D.~Silvermyr}
\author[a6]{G.~Simonetti\fnref{f32}}
\author[a9]{R.~Singaraju}
\author[a48]{R.~Singh}
\author[a9]{B.C.~Sinha}
\author[a57]{T.~Sinha}
\author[a61]{B.~Sitar}
\author[a76]{M.~Sitta}
\author[a59]{T.B.~Skaali}
\author[a1]{K.~Skjerdal}
\author[a50]{R.~Smakal}
\author[a4]{N.~Smirnov}
\author[a51]{R.~Snellings\fnref{f33}}
\author[a44]{C.~S{\o}gaard}
\author[a55]{A.~Soloviev}
\author[a109]{R.~Soltz}
\author[a97]{H.~Son}
\author[a101]{M.~Song}
\author[a6]{C.~Soos}
\author[a25]{F.~Soramel}
\author[a91]{M.~Spyropoulou-Stassinaki}
\author[a112]{B.K.~Srivastava}
\author[a63]{J.~Stachel}
\author[a79]{I.~Stan}
\author[a85]{G.~Stefanek}
\author[a6]{G.~Stefanini}
\author[a22]{T.~Steinbeck\fnref{f4}}
\author[a71]{E.~Stenlund}
\author[a64]{G.~Steyn}
\author[a27]{D.~Stocco}
\author[a28]{R.~Stock}
\author[a55]{M.~Stolpovskiy}
\author[a61]{P.~Strmen}
\author[a81]{A.A.P.~Suaide}
\author[a34]{M.A.~Subieta~V\'{a}squez}
\author[a108]{T.~Sugitate}
\author[a58]{C.~Suire}
\author[a3]{M.~\v{S}umbera}
\author[a24]{T.~Susa}
\author[a6]{D.~Swoboda}
\author[a98]{T.J.M.~Symons}
\author[a81]{A.~Szanto~de~Toledo}
\author[a61]{I.~Szarka}
\author[a1]{A.~Szostak}
\author[a91]{C.~Tagridis}
\author[a69]{J.~Takahashi}
\author[a58]{J.D.~Tapia~Takaki}
\author[a6]{A.~Tauro}
\author[a6]{M.~Tavlet}
\author[a75]{G.~Tejeda~Mu\~{n}oz}
\author[a6]{A.~Telesca}
\author[a18]{C.~Terrevoli}
\author[a19]{J.~Th\"{a}der}
\author[a70]{D.~Thomas}
\author[a19]{J.H.~Thomas}
\author[a68]{R.~Tieulent}
\author[a46]{A.R.~Timmins\fnref{f6}}
\author[a50]{D.~Tlusty}
\author[a6]{A.~Toia}
\author[a108]{H.~Torii}
\author[a6]{L.~Toscano}
\author[a14]{F.~Tosello}
\author[a92]{T.~Traczyk}
\author[a23]{D.~Truesdale}
\author[a32]{W.H.~Trzaska}
\author[a62]{A.~Tumkin}
\author[a88]{R.~Turrisi}
\author[a67]{A.J.~Turvey}
\author[a59]{T.S.~Tveter}
\author[a28]{J.~Ulery}
\author[a1]{K.~Ullaland}
\author[a84]{A.~Uras}
\author[a56]{J.~Urb\'{a}n}
\author[a86]{G.M.~Urciuoli}
\author[a84]{G.L.~Usai}
\author[a90]{A.~Vacchi}
\author[a43]{M.~Vala\fnref{f24}}
\author[a58]{L.~Valencia~Palomo}
\author[a63]{S.~Vallero}
\author[a51]{N.~van~der~Kolk}
\author[a70]{M.~van~Leeuwen}
\author[a6]{P.~Vande~Vyvre}
\author[a78]{L.~Vannucci}
\author[a75]{A.~Vargas}
\author[a99]{R.~Varma}
\author[a91]{M.~Vasileiou}
\author[a13]{A.~Vasiliev}
\author[a20]{V.~Vechernin}
\author[a60]{M.~Venaruzzo}
\author[a34]{E.~Vercellin}
\author[a75]{S.~Vergara}
\author[a113]{R.~Vernet}
\author[a70]{M.~Verweij}
\author[a94]{L.~Vickovic}
\author[a25]{G.~Viesti}
\author[a62]{O.~Vikhlyantsev}
\author[a64]{Z.~Vilakazi}
\author[a40]{O.~Villalobos~Baillie}
\author[a13]{A.~Vinogradov}
\author[a20]{L.~Vinogradov}
\author[a62]{Y.~Vinogradov}
\author[a82]{T.~Virgili}
\author[a9]{Y.P.~Viyogi}
\author[a43]{A.~Vodopyanov}
\author[a12]{K.~Voloshin}
\author[a46]{S.~Voloshin}
\author[a18]{G.~Volpe}
\author[a6]{B.~von~Haller}
\author[a19]{D.~Vranic}
\author[a56]{J.~Vrl\'{a}kov\'{a}}
\author[a37]{B.~Vulpescu}
\author[a1]{B.~Wagner}
\author[a50]{V.~Wagner}
\author[a45]{R.~Wan\fnref{f34}}
\author[a65]{D.~Wang}
\author[a63]{Y.~Wang}
\author[a65]{Y.~Wang}
\author[a72]{K.~Watanabe}
\author[a42]{J.P.~Wessels}
\author[a42]{U.~Westerhoff}
\author[a63]{J.~Wiechula}
\author[a59]{J.~Wikne}
\author[a42]{M.~Wilde}
\author[a42]{A.~Wilk}
\author[a85]{G.~Wilk}
\author[a26]{M.C.S.~Williams}
\author[a63]{B.~Windelband}
\author[a36]{H.~Yang}
\author[a13]{S.~Yasnopolskiy}
\author[a114]{J.~Yi}
\author[a65]{Z.~Yin}
\author[a72]{H.~Yokoyama}
\author[a114]{I.-K.~Yoo}
\author[a65]{X.~Yuan}
\author[a13]{I.~Yushmanov}
\author[a59]{E.~Zabrodin}
\author[a6]{C.~Zampolli}
\author[a43]{S.~Zaporozhets}
\author[a20]{A.~Zarochentsev}
\author[a105]{P.~Z\'{a}vada}
\author[a92]{H.~Zbroszczyk}
\author[a22]{P.~Zelnicek}
\author[a55]{A.~Zenin}
\author[a79]{I.~Zgura}
\author[a47]{M.~Zhalov}
\author[a65]{X.~Zhang\fnref{f1}}
\author[a65]{D.~Zhou}
\author[a15]{A.~Zichichi\fnref{f35}}
\author[a16]{G.~Zinovjev}
\author[a68]{Y.~Zoccarato}
\author[a16]{M.~Zynovyev}
%
\fntext[f1]{Also at Laboratoire de Physique Corpusculaire (LPC), Clermont Universit\'{e}, Universit\'{e} Blaise Pascal, CNRS--IN2P3, Clermont-Ferrand, France}
\fntext[f2]{Now at Centro Fermi -- Centro Studi e Ricerche e Museo Storico della Fisica ``Enrico Fermi'', Rome, Italy}
\fntext[f3]{Now at Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany}
\fntext[f4]{Now at Frankfurt Institute for Advanced Studies, Johann Wolfgang Goethe-Universit\"{a}t Frankfurt, Frankfurt, Germany}
\fntext[f5]{Now at Sezione INFN, Turin, Italy}
\fntext[f6]{Now at University of Houston, Houston, Texas, United States}
\fntext[f7]{Also at  Dipartimento di Fisica dell'Universit\'{a}, Udine, Italy }
\fntext[f8]{Now at SUBATECH, Ecole des Mines de Nantes, Universit\'{e} de Nantes, CNRS-IN2P3, Nantes, France}
\fntext[f9]{Now at Centro de Investigaci\'{o}n y de Estudios Avanzados (CINVESTAV), Mexico City and M\'{e}rida, Mexico}
\fntext[f10]{Now at Benem\'{e}rita Universidad Aut\'{o}noma de Puebla, Puebla, Mexico}
\fntext[f11]{Now at Laboratoire de Physique Subatomique et de Cosmologie (LPSC), Universit\'{e} Joseph Fourier, CNRS-IN2P3, Institut Polytechnique de Grenoble, Grenoble, France}
\fntext[f12]{Now at Institut Pluridisciplinaire Hubert Curien (IPHC), Universit\'{e} de Strasbourg, CNRS-IN2P3, Strasbourg, France}
\fntext[f13]{Now at Sezione INFN, Padova, Italy}
\fntext[f14]{ Deceased }
\fntext[f15]{Also at Division of Experimental High Energy Physics, University of Lund, Lund, Sweden}
\fntext[f16]{Also at  University of Technology and Austrian Academy of Sciences, Vienna, Austria }
\fntext[f17]{Also at European Organization for Nuclear Research (CERN), Geneva, Switzerland}
\fntext[f18]{Now at Oak Ridge National Laboratory, Oak Ridge, Tennessee, United States}
\fntext[f19]{Now at European Organization for Nuclear Research (CERN), Geneva, Switzerland}
\fntext[f20]{Also at Wayne State University, Detroit, Michigan, United States}
\fntext[f21]{Also at Frankfurt Institute for Advanced Studies, Johann Wolfgang Goethe-Universit\"{a}t Frankfurt, Frankfurt, Germany}
\fntext[f22]{Now at Research Division and ExtreMe Matter Institute EMMI, GSI Helmholtzzentrum f\"ur Schwerionenforschung, Darmstadt, Germany}
\fntext[f23]{Also at Fachhochschule K\"{o}ln, K\"{o}ln, Germany}
\fntext[f24]{Also at Institute of Experimental Physics, Slovak Academy of Sciences, Ko\v{s}ice, Slovakia}
\fntext[f25]{Now at Instituto de Ciencias Nucleares, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Mexico City, Mexico}
\fntext[f26]{Also at Laboratoire de Physique Subatomique et de Cosmologie (LPSC), Universit\'{e} Joseph Fourier, CNRS-IN2P3, Institut Polytechnique de Grenoble, Grenoble, France}
\fntext[f27]{Also at  "Vin\v{c}a" Institute of Nuclear Sciences, Belgrade, Serbia }
\fntext[f28]{Also at University of Houston, Houston, Texas, United States}
\fntext[f29]{Also at Department of Physics, University of Oslo, Oslo, Norway}
\fntext[f30]{Also at Variable Energy Cyclotron Centre, Kolkata, India}
\fntext[f31]{Now at Department of Physics, University of Oslo, Oslo, Norway}
\fntext[f32]{Also at Dipartimento Interateneo di Fisica `M.~Merlin' and Sezione INFN, Bari, Italy}
\fntext[f33]{Now at Nikhef, National Institute for Subatomic Physics and Institute for Subatomic Physics of Utrecht University, Utrecht, Netherlands}
\fntext[f34]{Also at Hua-Zhong Normal University, Wuhan, China}
\fntext[f35]{Also at Centro Fermi -- Centro Studi e Ricerche e Museo Storico della Fisica ``Enrico Fermi'', Rome, Italy}
\address[a1]{Department of Physics and Technology, University of Bergen, Bergen, Norway}
\address[a2]{Centro de Aplicaciones Tecnol\'{o}gicas y Desarrollo Nuclear (CEADEN), Havana, Cuba}
\address[a3]{Nuclear Physics Institute, Academy of Sciences of the Czech Republic, \v{R}e\v{z} u Prahy, Czech Republic}
\address[a4]{Yale University, New Haven, Connecticut, United States}
\address[a5]{Physics Department, Panjab University, Chandigarh, India}
\address[a6]{European Organization for Nuclear Research (CERN), Geneva, Switzerland}
\address[a7]{KFKI Research Institute for Particle and Nuclear Physics, Hungarian Academy of Sciences, Budapest, Hungary}
\address[a8]{Instituto de F\'{\i}sica, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Mexico City, Mexico}
\address[a9]{Variable Energy Cyclotron Centre, Kolkata, India}
\address[a10]{Department of Physics Aligarh Muslim University, Aligarh, India}
\address[a11]{Gangneung-Wonju National University, Gangneung, South Korea}
\address[a12]{Institute for Theoretical and Experimental Physics, Moscow, Russia}
\address[a13]{Russian Research Centre Kurchatov Institute, Moscow, Russia}
\address[a14]{Sezione INFN, Turin, Italy}
\address[a15]{Dipartimento di Fisica dell'Universit\`{a} and Sezione INFN, Bologna, Italy}
\address[a16]{Bogolyubov Institute for Theoretical Physics, Kiev, Ukraine}
\address[a17]{Frankfurt Institute for Advanced Studies, Johann Wolfgang Goethe-Universit\"{a}t Frankfurt, Frankfurt, Germany}
\address[a18]{Dipartimento Interateneo di Fisica `M.~Merlin' and Sezione INFN, Bari, Italy}
\address[a19]{Research Division and ExtreMe Matter Institute EMMI, GSI Helmholtzzentrum f\"ur Schwerionenforschung, Darmstadt, Germany}
\address[a20]{V.~Fock Institute for Physics, St. Petersburg State University, St. Petersburg, Russia}
\address[a21]{National Institute for Physics and Nuclear Engineering, Bucharest, Romania}
\address[a22]{Kirchhoff-Institut f\"{u}r Physik, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany}
\address[a23]{Department of Physics, Ohio State University, Columbus, Ohio, United States}
\address[a24]{Rudjer Bo\v{s}kovi\'{c} Institute, Zagreb, Croatia}
\address[a25]{Dipartimento di Fisica dell'Universit\`{a} and Sezione INFN, Padova, Italy}
\address[a26]{Sezione INFN, Bologna, Italy}
\address[a27]{SUBATECH, Ecole des Mines de Nantes, Universit\'{e} de Nantes, CNRS-IN2P3, Nantes, France}
\address[a28]{Institut f\"{u}r Kernphysik, Johann Wolfgang Goethe-Universit\"{a}t Frankfurt, Frankfurt, Germany}
\address[a29]{Laboratoire de Physique Subatomique et de Cosmologie (LPSC), Universit\'{e} Joseph Fourier, CNRS-IN2P3, Institut Polytechnique de Grenoble, Grenoble, France}
\address[a30]{Departamento de F\'{\i}sica de Part\'{\i}culas and IGFAE, Universidad de Santiago de Compostela, Santiago de Compostela, Spain}
\address[a31]{Oak Ridge National Laboratory, Oak Ridge, Tennessee, United States}
\address[a32]{Helsinki Institute of Physics (HIP) and University of Jyv\"{a}skyl\"{a}, Jyv\"{a}skyl\"{a}, Finland}
\address[a33]{Sezione INFN, Catania, Italy}
\address[a34]{Dipartimento di Fisica Sperimentale dell'Universit\`{a} and Sezione INFN, Turin, Italy}
\address[a35]{Centro Fermi -- Centro Studi e Ricerche e Museo Storico della Fisica ``Enrico Fermi'', Rome, Italy}
\address[a36]{Commissariat \`{a} l'Energie Atomique, IRFU, Saclay, France}
\address[a37]{Laboratoire de Physique Corpusculaire (LPC), Clermont Universit\'{e}, Universit\'{e} Blaise Pascal, CNRS--IN2P3, Clermont-Ferrand, France}
\address[a38]{Institute of Experimental Physics, Slovak Academy of Sciences, Ko\v{s}ice, Slovakia}
\address[a39]{Dipartimento di Fisica e Astronomia dell'Universit\`{a} and Sezione INFN, Catania, Italy}
\address[a40]{School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom}
\address[a41]{The Henryk Niewodniczanski Institute of Nuclear Physics, Polish Academy of Sciences, Cracow, Poland}
\address[a42]{Institut f\"{u}r Kernphysik, Westf\"{a}lische Wilhelms-Universit\"{a}t M\"{u}nster, M\"{u}nster, Germany}
\address[a43]{Joint Institute for Nuclear Research (JINR), Dubna, Russia}
\address[a44]{Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark}
\address[a45]{Institut Pluridisciplinaire Hubert Curien (IPHC), Universit\'{e} de Strasbourg, CNRS-IN2P3, Strasbourg, France}
\address[a46]{Wayne State University, Detroit, Michigan, United States}
\address[a47]{Petersburg Nuclear Physics Institute, Gatchina, Russia}
\address[a48]{Physics Department, University of Jammu, Jammu, India}
\address[a49]{Laboratori Nazionali di Frascati, INFN, Frascati, Italy}
\address[a50]{Faculty of Nuclear Sciences and Physical Engineering, Czech Technical University in Prague, Prague, Czech Republic}
\address[a51]{Nikhef, National Institute for Subatomic Physics, Amsterdam, Netherlands}
\address[a52]{Centro de Investigaciones Energ\'{e}ticas Medioambientales y Tecnol\'{o}gicas (CIEMAT), Madrid, Spain}
\address[a53]{University of Houston, Houston, Texas, United States}
\address[a54]{Moscow Engineering Physics Institute, Moscow, Russia}
\address[a55]{Institute for High Energy Physics, Protvino, Russia}
\address[a56]{Faculty of Science, P.J.~\v{S}af\'{a}rik University, Ko\v{s}ice, Slovakia}
\address[a57]{Saha Institute of Nuclear Physics, Kolkata, India}
\address[a58]{Institut de Physique Nucl\'{e}aire d'Orsay (IPNO), Universit\'{e} Paris-Sud, CNRS-IN2P3, Orsay, France}
\address[a59]{Department of Physics, University of Oslo, Oslo, Norway}
\address[a60]{Dipartimento di Fisica dell'Universit\`{a} and Sezione INFN, Trieste, Italy}
\address[a61]{Faculty of Mathematics, Physics and Informatics, Comenius University, Bratislava, Slovakia}
\address[a62]{Russian Federal Nuclear Center (VNIIEF), Sarov, Russia}
\address[a63]{Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany}
\address[a64]{Physics Department, University of Cape Town, iThemba Laboratories, Cape Town, South Africa}
\address[a65]{Hua-Zhong Normal University, Wuhan, China}
\address[a66]{Secci\'{o}n F\'{\i}sica, Departamento de Ciencias, Pontificia Universidad Cat\'{o}lica del Per\'{u}, Lima, Peru}
\address[a67]{Physics Department, Creighton University, Omaha, Nebraska, United States}
\address[a68]{Universit\'{e} de Lyon, Universit\'{e} Lyon 1, CNRS/IN2P3, IPN-Lyon, Villeurbanne, France}
\address[a69]{Universidade Estadual de Campinas (UNICAMP), Campinas, Brazil}
\address[a70]{Nikhef, National Institute for Subatomic Physics and Institute for Subatomic Physics of Utrecht University, Utrecht, Netherlands}
\address[a71]{Division of Experimental High Energy Physics, University of Lund, Lund, Sweden}
\address[a72]{University of Tsukuba, Tsukuba, Japan}
\address[a73]{Sezione INFN, Cagliari, Italy}
\address[a74]{Centro de Investigaci\'{o}n y de Estudios Avanzados (CINVESTAV), Mexico City and M\'{e}rida, Mexico}
\address[a75]{Benem\'{e}rita Universidad Aut\'{o}noma de Puebla, Puebla, Mexico}
\address[a76]{Dipartimento di Scienze e Tecnologie Avanzate dell'Universit\`{a} del Piemonte Orientale and Gruppo Collegato INFN, Alessandria, Italy}
\address[a77]{Instituto de Ciencias Nucleares, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Mexico City, Mexico}
\address[a78]{Laboratori Nazionali di Legnaro, INFN, Legnaro, Italy}
\address[a79]{Institute of Space Sciences (ISS), Bucharest, Romania}
\address[a80]{Institute of Physics, Bhubaneswar, India}
\address[a81]{Universidade de S\~{a}o Paulo (USP), S\~{a}o Paulo, Brazil}
\address[a82]{Dipartimento di Fisica `E.R.~Caianiello' dell'Universit\`{a} and Gruppo Collegato INFN, Salerno, Italy}
\address[a83]{Sezione INFN, Bari, Italy}
\address[a84]{Dipartimento di Fisica dell'Universit\`{a} and Sezione INFN, Cagliari, Italy}
\address[a85]{Soltan Institute for Nuclear Studies, Warsaw, Poland}
\address[a86]{Sezione INFN, Rome, Italy}
\address[a87]{Faculty of Engineering, Bergen University College, Bergen, Norway}
\address[a88]{Sezione INFN, Padova, Italy}
\address[a89]{Institute for Nuclear Research, Academy of Sciences, Moscow, Russia}
\address[a90]{Sezione INFN, Trieste, Italy}
\address[a91]{Physics Department, University of Athens, Athens, Greece}
\address[a92]{Warsaw University of Technology, Warsaw, Poland}
\address[a93]{Universidad Aut\'{o}noma de Sinaloa, Culiac\'{a}n, Mexico}
\address[a94]{Technical University of Split FESB, Split, Croatia}
\address[a95]{Yerevan Physics Institute, Yerevan, Armenia}
\address[a96]{University of Tokyo, Tokyo, Japan}
\address[a97]{Department of Physics, Sejong University, Seoul, South Korea}
\address[a98]{Lawrence Berkeley National Laboratory, Berkeley, California, United States}
\address[a99]{Indian Institute of Technology, Mumbai, India}
\address[a100]{Institut f\"{u}r Kernphysik, Technische Universit\"{a}t Darmstadt, Darmstadt, Germany}
\address[a101]{Yonsei University, Seoul, South Korea}
\address[a102]{Zentrum f\"{u}r Technologietransfer und Telekommunikation (ZTT), Fachhochschule Worms, Worms, Germany}
\address[a103]{California Polytechnic State University, San Luis Obispo, California, United States}
\address[a104]{China Institute of Atomic Energy, Beijing, China}
\address[a105]{Institute of Physics, Academy of Sciences of the Czech Republic, Prague, Czech Republic}
\address[a106]{University of Tennessee, Knoxville, Tennessee, United States}
\address[a107]{Dipartimento di Fisica dell'Universit\`{a} `La Sapienza' and Sezione INFN, Rome, Italy}
\address[a108]{Hiroshima University, Hiroshima, Japan}
\address[a109]{Lawrence Livermore National Laboratory, Livermore, California, United States}
\address[a110]{Budker Institute for Nuclear Physics, Novosibirsk, Russia}
\address[a111]{Physics Department, University of Rajasthan, Jaipur, India}
\address[a112]{Purdue University, West Lafayette, Indiana, United States}
\address[a113]{Centre de Calcul de l'IN2P3, Villeurbanne, France }
\address[a114]{Pusan National University, Pusan, South Korea}
% End of author list
